QoS-Aware Placement of Deep Learning Services on the Edge with Multiple Service Implementations

Mobile edge computing pushes computationally-intensive services closer to the user to provide reduced delay due to physical proximity. This has led many to consider deploying deep learning models on the edge -- commonly known as edge intelligence (EI). EI services can have many model implementations that provide different QoS. For instance, one model can perform inference faster than another (thus reducing latency) while achieving less accuracy when evaluated. In this paper, we study joint service placement and model scheduling of EI services with the goal to maximize Quality-of-Servcice (QoS) for end users where EI services have multiple implementations to serve user requests, each with varying costs and QoS benefits. We cast the problem as an integer linear program and prove that it is NP-hard. We then prove the objective is equivalent to maximizing a monotone increasing, submodular set function and thus can be solved greedily while maintaining a (1-1/e)-approximation guarantee. We then propose two greedy algorithms: one that theoretically guarantees this approximation and another that empirically matches its performance with greater efficiency. Finally, we thoroughly evaluate the proposed algorithm for making placement and scheduling decisions in both synthetic and real-world scenarios against the optimal solution and some baselines. In the real-world case, we consider real machine learning models using the ImageNet 2012 data-set for requests. Our numerical experiments empirically show that our more efficient greedy algorithm is able to approximate the optimal solution with a 0.904 approximation on average, while the next closest baseline achieves a 0.607 approximation on average.

==> fig/tex/realworld-boxen.tex <==
\begin{figure}
    \centering
% 	\includegraphics[width=0.775\linewidth]{fig/plots/real-world/qos-kde}
	\includegraphics[width=0.775\linewidth]{fig/plots/real-world/qos-boxen}
    \caption{QoS CDF plot in real-world scenario.}
    \label{fig:realworld_qos}
\end{figure}

==> fig/tex/realworld-placements.tex <==
\begin{figure}
    \centering
% 	\includegraphics[width=0.775\linewidth]{fig/plots/real-world/qos-kde}
	\includegraphics[width=0.775\linewidth]{fig/plots/real-world/placement-bar}
    \caption{QoS CDF plot in real-world scenario.}
    \label{fig:realworld_placements}
\end{figure}

==> fig/tex/realworld.tex <==
\begin{figure}
    \centering
% 	\includegraphics[width=0.775\linewidth]{fig/plots/real-world/qos-kde}
	\includegraphics[width=0.775\linewidth]{fig/plots/real-world/qos-ecdf}
    \caption{QoS CDF plot in real-world scenario.}
    \label{fig:realworld_qos}
\end{figure}

==> pseudocode/EGP_v1.tex <==
\begin{algorithm}[t]
	\footnotesize
	%%
    % Define the input/output keywords.
    %%
    \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
    \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
    
    %%
    % Input and output for the algorithm.
    %%
    \Input{Input parameters of~\eqref{eq:PIES}}
    \Output{Service placement $(\textbf{x})$}
    
	Init $\textbf{x} \gets (x_e^{sm}=0)_{\forall e\in\edges, s\in\services, m\in\model}$\;
    
    \ForEach{edge $e\in\edges$}{
    	usedStorage $\gets 0$\;
    	
		$v \gets \textbf{new}$ hash data structure (default values $= 0$)\;

		\ForEach{$u \in \users_e$}{
			\ForEach{$m \in \model_{s_u}$}{
				\If{$r_{s_um} + \text{usedStorage} \leq R_e$}{
					% $v_{s^*m} \gets v_{s_um} + \frac{1}{r_{s_um}}Q(u,s_u,m)$\;
					$v_{s_um} \gets v_{s_um} + \frac{1}{r_{s_um}}Q(u,s_u,m)$\;
				}
			}
		}
		
		satisfied $\gets \{\}$\;
		\While{$|\users_e\setminus\text{satisfied}| > 0$ and $v$ is not empty}{
			$(s^*, m^*) \gets \argmax_{(s,m)\in\SM}\big\{v_{sm}\big\}$\;
			\If{$r_{s^*m^*} + \text{usedStorage} > R_e$}{
				Remove $(s^*,m^*)$ key-value pair from $v$\;
				\textbf{continue}\;
			}
			
			newlySatisfied $\gets \{\}$\;
			\ForEach{$u \in \users_e \setminus$ satisfied}{
				\If{$A_{s^* m^*} \geq \alpha_u$ \textbf{or} $D_{s^*m^*}(u) \leq \delta_u$}{
					$\text{newlySatisfied} \gets \text{newlySatisfied} \cup \{u\}$\;
				}
			}
			
			\If{$|\text{newlySatisfied}| = 0$}{
				$u^{*} \gets \argmin_{u\in\users_e\setminus\text{satisfied}}$ $ \Big\{ \sqrt{(\alpha_u - A_{s^{*}m^{*}})^2 + (\delta_u - D_{s^{*}m^{*}}(u))^2} \Big\}$\;
				$\text{newlySatisfied} \gets \text{newlySatisfied} \cup \{u^{*}\}$\; 
			}
			
			\ForEach{$u \in \text{newlySatisfied}$}{
				\ForEach{$m \in \model_{s_u}$}{
					$v_{s^*m} \gets v_{s^*m} - \frac{1}{r_{s^*m}}Q(u,s^*,m)$\;
				}
			}
			
			$x_{e}^{s^*m^*} \gets 1$\;
			$\text{usedStorage} \gets \text{usedStorage} + r_{s^*m^*}$\;
			$\text{satisfied} \gets \text{satisfied} \cup \text{newlySatisfied}$\;
			Delete $v_{s^*m^*}$\;
		}
    }    
    \Return \textbf{x}\;

\caption{Efficient Greedy Placement~(EGP)}
%\caption{Greedy Service Model Placement}
\label{alg:greedy-placement}
\end{algorithm}

==> sections/old_experiments.tex <==
To solve the MSIP problem, we show that our greedy algorithm (described in Algorithm~\ref{alg:greedy}) demonstrates high efficacy and efficient runtime performance. Further, to demonstrate the significance of its performance, we compare it against a slew of baseline algorithms. We consider two cases: (1) General Case and (2) NN Special Case. 
%The former case is more interested in the more abstract view of the MSIP problem presented in Section~\ref{sec:MSIP} while the latter is interested in the DNN-, PNN-, and SNN-specific version of the problem presented in Section~\ref{sec:arch-MSIP}. We are interested in the latter case to better understand, at a high level, which scenarios make certain model types for ANNs more useful and the like. We also investigate problems related to distribution of model placement and scheduling in the NN Special Case to provide insight for when DNNs, PNNs, and SNNs might be useful.

% \subsection{Parameter Setup}
\textbf{Parameter Setup.}
Unless specified otherwise, we consider cases where $|\edges|=10$, $|\users|=1000$, $|\services|=100$, and, in the General Case, $|\model|=10$. Communication capacities for edge clouds are set to be $K_e=5~\text{MHz};(\forall e\in\edges)$. Computation and storage capacities are randomly and uniformly sampled from the ranges $[0.4~\text{GHz}, 0.6~\text{GHz}, \cdots, 1.0~\text{GHz}]$ and $[10, 11, \cdots, 100]$ (respectively). Storage costs for service models are uniformly sampled from $[1, 2, \cdots, 5]$. User accuracy tolerance thresholds (unless specified) are sampled from a normal distribution with a mean of $\sigma=0.75$ and a standard deviation of $0.125$. Model accuracy scores are generated from the same distribution. User delay tolerance thresholds (in seconds) are generated from a normal distribution with a mean of $\sigma=1.0$ and a standard deviation of $5$. All randomly sampled values for accuracy tolerance and delay tolerance are confined to their legal ranges of $(0, 1.0)$ and $[0.0, \tau_{\max}]$, respectively, where $\tau_{\max}=240$~seconds. \draft{We set $\tau_{\max}$ to be so large to accomodate rare cases where computed completion time in the NN Special Case are exceptionally high and to maintain a normalized range.} The maximum distance value $dist_{\max}=100$~meters and the 
% \hana{what is this bps here? maximum bps? maximum communication capacity?}
data transmission rate to the central cloud $bps_c=0.1~\text{MHz}$. For the General Case, the communication and computation costs for service models are both uniformly and randomly sampled from a range of $[10^3, 10^5]$. For the NN Special Case, each service first has a randomly generated DNN topology with a random number of layers belonging to the range $[10, 50]$ and with each layer consisting of a uniformly sampled number of neurons belonging to the range $[10^1, 10^4]$. 
% \hana{why this is relevant here? i didnt see any plot that compares those activation functions? i think you should at least mention that,otherwise they may look for results with different activations.} 
% \nathaniel{Do you think it would be easier to simply forego explicitly naming the activation functions and instead say, "computation costs associated with activation functions for each layer under our framework are randomly generated from..."?} 
Computation costs associated with each layer to represent activation function costs are assigned randomly ranging from [10,90].
% For the activation functions, we consider the following: I/O, convolutional, max pooling, fully connected, sigmoid, tanh, ReLU, leaky-ReLU, parameterized-ReLU, softmax, and swish. Each of these is provided a hard-coded computational cost based on intuition and experimentation ranging from 10 to 90. 
This parameter setup was chosen after extensive and exhaustive experimentation and sensitivity analysis. A more thorough analysis of this model and the parameters chosen is beyond the scope of this paper.




% \subsection{Baseline Algorithms}
\textbf{Baselines.}
For brevity, we refer to Greedy and Greedy-Random as \emph{greedy placement} algorithms. Our baselines for comparison are the following.
\underline{Optimal:} Serves as an upper bound using MSIP's ILP implemented with IBM's CPLEX solver~\cite{manual1987ibm}.
% 
\underline{Dynamic Knapsack:} A modified version of the dynamic programming solution to the \textsc{0/1 Knapsack} problem~\cite{dynamic_solution} to better fit the placement portion of the MSIP problem. The asymptotic runtime is $O(|\edges|\cdot(|\services||\model|(\log_2(|\services||\model|) + R^{*})))$ where $R^{*}=\max_{e\in\edges}(R_e)$. Algorithm~\ref{alg:greedy-scheduling} is used for scheduling. We adapt this algorithm by setting values for service models to be equal to the summation of expected QoS each provide to all users.
% 
\underline{Greedy-Random:} Greedy service placement from Algorithm~\ref{alg:greedy-placement} and random model scheduling for each user.
% 
\underline{Random-Greedy:} Random service placement and greedy model scheduling using Algorithm~\ref{alg:greedy-scheduling}.
% 
\underline{Random:} Random placement and model scheduling.

% \subsection{Experimental Results}
% \subsubsection{Total Quality-of-Service (QoS)}

%%
% FIGURE: TOTAL QOS AND ALGORITHM RUNTIMERESULTS.
%%
\begin{figure}
	\centering
	%% Total QoS
	\includegraphics[width=0.48\linewidth]{data/QoS-Experiment/gen-qos}  %% General Case
	\includegraphics[width=0.48\linewidth]{data/QoS-Experiment/arch-qos} %% NN Special Case
	%% Algorithm Runtime
	\subfloat[General Case\label{fig:gen-runtime}]{\includegraphics[width=0.48\linewidth]{data/QoS-Experiment/gen-time}} %% General Case
	\subfloat[NN Special Case\label{fig:arch-runtime}]{\includegraphics[width=0.48\linewidth]{data/QoS-Experiment/arch-time}} %% NN Special Case
	\caption{Total QoS and algorithm runtime as $|\users|$ increases. Error bars correspond with $\pm$ 1 standard deviation.}
	\label{fig:total_qos}
\end{figure}

\textbf{Experimental Results.}
In Figure~\ref{fig:total_qos}, we see the results of an experiment over 100 Monte-Carlo runs in both the General Case and the NN Special Case where each algorithm attempts to maximize the objective function (i.e., maximize total QoS) as the number of users increases. It is clear that both greedy placement algorithms are able to attain total QoS incredibly close to the optimal solution. What is compelling is the fact that the Knapsack solution notably underperforms with regard to finding a near-optimal solution. Our intuition for this is due to the multi-implementation nature of MSIP. This is likely due to the values of each service model in the MSIP problem functionally being non-static (i.e., if you pick a model for a service, the values of the other models for the same service degrade). This is due to the reality that the ``values" for service models is the net gain acquired in terms of total QoS. If a user can be served with an unsatisfactory model, they will still provide \emph{some} QoS, even if it is not maximal. As a result, other models for their service naturally degrade. So, while the dynamic program for the 0/1 Knapsack problem can be used to solve that problem in pseudo-polynomial time~\cite{dynamic_solution}, it underperforms in this problem for this reason. Another interesting observation is that the scheduling policy (i.e., Greedy vs. Greedy-Random) provide insignificant improvement to the overall total QoS in the NN Special Case --- highlighting the importance of placement over scheduling in the context of our model. This is likely due to there being, at most, three model types available in the NN Special Case, thus minimizing room for error. 
Additionally, we find that the runtime of our greedy algorithm scales well and outdoes both the optimal solver and the dynamic knapsack. It is important to note that the runtime of the dynamic knapsack solution is intrinsically tied to storage costs/capacities --- leading us to choose smaller capacities and costs for simulation. 
Figure~\ref{fig:qos_norm} also highlights the runtime performance of our algorithm where each point represents the average QoS across all users and the algorithm runtime.
% 
Next, we compare the average similarity between our algorithm and the baselines with the optimal solution. We consider the ratio $\frac{\text{QoS}_a}{\text{QoS}_{\text{opt}}}$ where $\text{QoS}_a$ is the objective value given decisions of algorithm/baseline $a$ and $\text{QoS}_{\text{opt}}$ is the objective value given the optimal solution. We average this ratio overall 100 trials performed for the QoS experiments to assess how close to optimal our greedy solution is. In Table~\ref{tab:similarity}, we observe that solutions involving our greedy placement algorithm outperform all other baselines, with Greedy nearly matching the optimal solution in the General Case.



%%
% FIGURE: QOS NORMALIZED PLOTS.
%%
\begin{figure}
	\centering
	%% General Case.
	\subfloat[General Case\label{fig:gen-norm}]{\includegraphics[width=0.48\linewidth]{data/QoS-Experiment/norm}}
	%% NN Special Case.
	\subfloat[NN Special Case\label{fig:arch-norm}]{\includegraphics[width=0.48\linewidth]{data/QoS-Experiment/norm-arch}}
	\caption{Average QoS in each Monte-Carlo run, i.e., $\frac{1}{|\users|}(\text{Total QoS})$, plotted against Algorithm's runtime.}
	\label{fig:qos_norm}
\end{figure}

\begin{table}
\centering
\footnotesize
\caption{Similarity Ratio Comparison.}
\label{tab:similarity}
\begin{tabular}{rcc}
	\toprule
	& \multicolumn{2}{c}{Average Similarity to Optimal} \\
	\cmidrule{2-3}
	Algorithm & General Case & NN Special Case \\
	\midrule
	Greedy        & \textbf{0.991163} & \textbf{0.905163} \\
	Knapsack      & 0.601003          & 0.699283          \\
	Greedy-Random & 0.772403          & \textbf{0.900425} \\
	Random-Greedy & 0.367579          & 0.428092          \\
	Random        & 0.379301          & 0.440481          \\
	\bottomrule
\end{tabular}	
\end{table}


%alg      num_place_sm    num_scheduled_sm    expected_QoS    alg_runtime
%-----  --------------  ------------------  --------------  -------------
%Opt               131                 344        170.204   75061.9
%Gr                130                 335        164.973       0.448382
%KS                120                 134         65.6347      3.30509
%RR                 57                  66         32.4547      0.0112009

\new{
\begin{table}
	\centering
	\caption{Simple algorithm comparison.}
	\label{tab:simple_comparison}
	\begin{tabular}{rcccc}
		\toprule
		Algorithm & $\sum x_{e}^{sm}$ & $\sum y_{u}^{m}$ & QoS & Alg. Runtime \\
		\midrule
		Optimal       & 131 & 344 & 170.204  &  20 hrs, 51 mins, 01 sec \\
		Greedy        & 130 & 335 & 164.973  & 0.448 sec \\
		Knapsack      & 120 & 134 &  65.6347 & 3.305 sec \\
		Ran-Ran &  57 &  66 &  32.4547 & 0.0112 sec \\
		\bottomrule
	\end{tabular}
\end{table}
}


%\subsubsection{Algorithmic Running Time}
%In Figure~\ref{fig:algorithm_tuntimes},
%%In Table~\ref{tab:runtime}, 
%we see the average runtime for each considered algorithm over 100 Monte-Carlo runs for both the General Case and NN Special Case. We see that our algorithm performs notably efficiently in comparison to both the optimal solver and the dynamic programming solution for the 0/1 Knapsack problem under both experimental cases. It should be noted, however, that we chose conservative storage capacities and costs for edge clouds and service models (respectively) to make the overall runtime for the knapsack solution reasonable.
%It is important to note that there is a notable reduction in running time from the General Case to the NN Special Case. This is likely due to the simple fact that we considered more model types for the General Case (i.e., $|\model|=10$) in comparison to the NN Special Case (i.e., $|\model|=3$). Nonetheless, our algorithm still solidly outperforms both the optimal solution and the knapsack solution in both cases.

% \subsubsection{Average QoS vs. Algorithm Runtime}
% Figure~\ref{fig:qos_norm} provides a holistic view of how the tested solutions compare in terms of maximizing the average QoS provided to users in a single Monte-Carlo run. We see that the optimal solver provides high average QoS but at the expense of inordinate runtime in both the General and NN Special Cases. In the latter, we see an anomaly of when the optimal solver takes more than 80 seconds to make its decisions. In contrast, we see that our greedy placement algorithms perform comparably in terms of delivering high average QoS, but with the benefit of consistent minimal runtime. Additionally, the Knapsack baseline in both cases is notably falling short of our greedy placement algorithms in both average QoS and runtime.


\begin{comment}
		\subsubsection{Placement and Scheduling Density}
		
		\begin{figure}
			\centering
			%% Placement KDE figure.
			\includegraphics[width=\linewidth]{data/ThresholdPlacement-experiment/kde-threshold-placement.pdf}
			\caption{Threshold Placement KDE using Optimal.}
			\label{fig:kde-threshold-placement}
			
			\smallbreak
			
			%% Scheduling KDE figure.
			\includegraphics[width=\linewidth]{data/ThresholdScheduling-experiment/kde-threshold-scheduling}
			\caption{Threshold Scheduling KDE using Optimal.}
			\label{fig:kde-threshold-scheduling}
		\end{figure}
		
		In the NN Special Case, we are interested in understanding how user QoS parameters impact the placement and scheduling of DNNs, PNNs, and SNNs under our model. This is to help find some high-level intuition as to which scenarios each type might be more appealing for both placement and scheduling in the goal of maximizing QoS. In Figures~\ref{fig:kde-threshold-placement} and~\ref{fig:kde-threshold-scheduling}, we see \draft{bivariate \emph{kernel density estimate} (KDE) plots} visualizing where placement and scheduling decisions (respectively) cluster for the three considered model types. 
		\draft{Briefly, these plots visualize ``clusters" of where decisions to place and schedule model types are being made based on the x- and y-axes --- darker corresponds to more occurrences of placement and scheduling decisions being made.}
		For these experiments, we set the x-axis ($\alpha_u$) and y-axis ($\tau_u$) uniformly for all users to be $\alpha_u=0.0, 0.1, \cdots, 1.0$ and $\tau_u = 0, 1, \cdots, 10$ (respectively).
		In Figure~\ref{fig:kde-threshold-placement}, we see that the placement of PNNs appears to be largely uniform relative to DNNs and SNNs. DNNs cluster in a seemingly linear fashion between both accuracy and delay tolerance thresholds. Interestingly, SNNs seem to only be placed in the case where users have high minimum accuracy tolerance thresholds.
		In Figure~\ref{fig:kde-threshold-scheduling}, a similar pattern is observed for SNNs --- the most density is seen where users have a high accuracy threshold. The inverse is seen for the PNNs: we see greater density for scheduling for PNNs in the cases where user minimal accuracy is low and density gradually decreases as user minimal accuracy thresholds increase. We see that DNNs have a few points of clusters throughout the entire space, most prominently in the bottom right corner where accuracy demands are high and delay tolerance is low. 
		\draft{It should be clarified that our KDE plots do not show the lowest shade to make the visualized shape more distinct. As such, there are scheduling decisions made in cases where it appears that no models have been placed. This is only a result of that visualization detail for clarity.}
		
		In conjunction with these plots, we also provide 
		%Figures~\ref{fig:model-dist-placement} and~\ref{fig:model-dist-scheduling} 
		Figure~\ref{fig:model-dist} 
		to show the breakdown of all considered algorithms for both placement and scheduling (respectively) using the standard parameters described earlier and $|\users|=1000$. What is interesting is that the placement/scheduling of our near-optimal solution varies greatly from the optimal solution. This is interesting given how similar the greedy placement algorithms perform in terms of total QoS in comparison with the optimal solution.
		
		%%
		% FIGURE: MODEL DISTRIBUTION EXPERIMENT
		%%
		\begin{figure}
			\centering
			%% Placement model-wise distribution.
			\includegraphics[width=\linewidth]{data/ModelDist-Experiment/placement-plot}
			
			%% Scheduling model-wise distribution.
			\includegraphics[width=\linewidth]{data/ModelDist-Experiment/scheduling-plot}
			
			\caption{Breakdown of decisions for placement (top) and scheduling (bottom) made by each Algorithm in the NN Special Case, $(|\users|=1000)$.}
			\label{fig:model-dist}
		\end{figure}
\end{comment}

%%
% FIGURE: DROPPED RATE EXPERIMENT
%%
\begin{figure}[t]
	\centering
	\subfloat[General Case\label{fig:gen-dropped}]{\includegraphics[width=0.5\linewidth]{data/DroppedRate-Experiment/dropped}}
	%
	\subfloat[NN Special Case\label{fig:arch-dropped}]{\includegraphics[width=0.5\linewidth]{data/DroppedRate-Experiment/arch-dropped}}
	%
	\caption{Percent of users dropped (i.e., offloaded to the cloud). Error bars correspond with $\pm$ 1 standard deviation.}
	\label{fig:dropped}
\end{figure}



\textbf{User Drop Rates.}
We investigate the percentages of dropped users (i.e., served by the central cloud) in both the General and NN Special Cases. In Figures~\ref{fig:gen-dropped} and~\ref{fig:arch-dropped}, we observe little changes across the two cases. The greedy placement algorithms closely match the optimal solution. The optimal solution approaches 40\% of users dropped to be served by the cloud as the number of users increases. 
This is in stark contrast to roughly 60\% and 80\% of requests dropped for the Knapsack and Random placement solutions, respectively.
% \hana{somewhere in this paragraphmention what is the shade around curves in those plots showing.}
%This is interesting because, under our model, if there is \emph{any} model placed on the edge that can service a user's request for a particular service, then it will be used in lieu of the cloud.

\textbf{Distribution of placement decision.} In Figure~\ref{fig:kde_placement}, we plot the KDE of placement decisions made in the NN Special Case for a given value of accuracy and delay threshold parameters, ($\alpha_u$ and $\tau_u$). The optimal solver is run for experiments over all combinations when $\alpha_u = 0.0, 0.1, \cdots, 1.0\;(\forall u \in \users)$ and $\tau_u=0, 1, \cdots, 10\;(\forall u \in \users)$. Darker colors correspond with more placement decisions for that respective model type around those parameters.
% \hana{maybe say what are the value of those parameters here again}.
% \hana{this next sentence is not complete. you should again highlight that given the penalty of sending to the cloud is small and equal to $\theta=0.05$}
This visualization suggests that, under our high-level framework for ANN architectures, SNNs are more commonly placed when users have high-accuracy demands assuming the multiplicative penalty for extra communication with the central cloud is small, e.g., $\theta=0.05$. Also, PNNs are more uniformly placed under all scenarios --- likely due to their smaller resource footprint.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{data/ThresholdPlacement-experiment/kde-threshold-placement.pdf}
    \caption{Optimal placement decision KDE plots as fixed threshold parameters increase in the NN Special Case.}
    \label{fig:kde_placement}
\end{figure}

==> sections/special_case.tex <==
%%
% FIGURE: ARTIFICIAL NEURAL NETWORKS
%%
\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{fig/ANN}
	\caption{The three considered ANN model types. The DNN, is the original architecture with the PNN generated with a pruning rate $\gamma=0.5$ and the SNN is split with $\rho=0.5$. }
	\label{fig:ANN-architecture}
\end{figure}


\section{Special Case: Neural Network Models}
\label{sec:arch-MSIP}

%\textbf{Edge Intelligence.}
% Due to the growing prominence of MEC, there has been much interest in deploying complex machine learning models to the edge of the network for reduced latency, increased reliability, and less reliance on a centralized location~\cite{EI_survey1, EI_survey2}. 
Machine learning (ML)-based applications is growing in the recent years. Given the popularity of ML models for different IoT applications, an emerging research area is currently focused on efficient employment of ML models at the edge. 
%is finding lighter implementations of ML models that can achieve reasonable accuracy and therefore, usable for small devices, such as those at the edge of the networks.
Due to the relative hardware limitations of edge clouds, approaches to reducing computational cost associated with ML models has been investigated for MEC~\cite{EI_survey1, EI_survey2, EI_fog}. One recent approach for model training and model inference on the edge is \emph{split learning} (SL) where a portion of a model's architecture is run on the edge and the other portion run on the central cloud~\cite{SL_1, SL_2}. Another proposal for providing less complex models on the edge is that of neural network pruning, where the original neural network's architecture is condensed by removing layers and neurons to make the task of inference/training less computationally expensive~\cite{prune1, prune2, prune3, prune4}.
Both split learning and pruned neural networks can be seen as two different implementations of a deep neural network.
Considering the proposed MSIP problem in Section~\ref{sec:MSIP} is fairly general, we investigate a more explicit special case of our problem using a high-level framework for representing \emph{artificial neural networks} (ANNs) as services. We then use this framework to formulate attained accuracy scores and expected completion times for the following ANN model types: \emph{(i)} \emph{deep neural networks} (DNNs), \emph{(ii)} \emph{pruned neural networks} (PNNs), and \emph{(iii)} \emph{split neural networks} (SNNs).\footnote{For simplicity, we will only consider \emph{sequential} ANNs for this work --- where the precedence and order of the layers are linear and no cycles exist.} 
Refer to Figure~\ref{fig:ANN-architecture} for a visual representation of the components of an ANN for this work.



\subsection{Modeling ANN Types}
Here, we briefly summarize our approach to modeling sequential DNNs, PNNs, and SNNs in terms of the computational and communication costs, as well as the accuracy performance they provide relative to one another.
\change{Our assumption in the special case is that the set of services $\services$ are all implemented with $|\model|=3$ separate model types: DNN, PNN, and SNN.} 
%Due to the increasing use of deep learning for complex problems (e.g., video classification, photo recognition, image segmentation, and so on), we decided to focus on \emph{deep neural networks} (DNNs) as the baseline and then consider two genres of neural networks more amenable to resource-constrained systems: \emph{pruned neural networks} (PNNs) and \emph{split neural networks} (SNNs). The need to consider some representation for individual architectures will be elaborated upon in Section~\ref{sec:arch-QoS}.


\subsubsection{Deep Neural Networks (DNNs)}
Sequential DNNs start with an input layer, followed by a sizable number of hidden layers, and then a single output layer. At a high level, each layer is equipped with a number of neurons and an activation function (e.g., tanh, ReLU, and sigmoid). The number of neurons varies greatly depending on the problem. For instance, the number of neurons in the input layer that accepts an image of 500 by 500 pixels is $500\times500\times3=750,000$ --- the three comes from a red, green, and blue (RGB) value for each pixel. To model that, we consider a vector $\ell^{sm}$ where $\ell_i^{sm}$ represents the number of neurons in the $i^{th}$ layer. 
\draft{We denote the number of layers in a given architecture as $N^{sm}$ where the following must hold: $N^{sm} \geq 2$ because an ANN must minimally have an input and an output layer.} 
Additionally, we consider a column vector $\beta^{sm}$ where $\beta_i^{sm}$ represents the number of CPU cycles needed to run the activation function for each neuron in the $i^{th}$ layer. The following condition must hold, $|\ell^{sm}|\equiv|\beta^{sm}|\;(\forall (s,m)\in\services\times\model)$. 
For simplicity, service models where $m=1$ are considered as DNNs in this version of the MSIP problem.


\subsubsection{Pruned Neural Networks (PNNs)}
Neural network pruning is an area of interest with the goal of better understanding which parts of a complex DNN can be removed without greatly impacting the model's efficacy. The notion of pruned neural networks has attracted attention in the context of MEC due to their reduced computational complexity. PNNs can have several layers from their original model removed and will even have a reduced number of neurons in each layer, aside from the output layer~\cite{prune1}. With that said, we consider a hyper-parameter $\gamma\in(0,1)$ that anneals the number of layers and the numbers of neurons in each layer of its corresponding DNN. 
For simplicity, service models where $m=2$ are considered as PNNs in this version of the MSIP problem.
First, we consider the number of neurons in each layer in the PNN to be $\ell_i^{s2}=\lceil\gamma\cdot\ell_i^{s1}\rceil\; (\forall i \in \ell^{s1}, \forall s\in\services)$, where $\ell_i^{s1}$ is the number of neurons of the $i^{th}$ layer of the original DNN model. We then prune the number of hidden layers at random.
More explicitly, let the number of layers $N^{s2} = \lceil\gamma(N^{s1} - 2)\rceil + 2\; (\forall s\in\services)$ where $N^{s1}-2$ is the number of hidden layers in the DNN which is multiplied by the pruning rate $\gamma$ and then added by 2 for the input and output layers.
Let storage costs $r_{s2} = \lceil \gamma \cdot r_{s1} \rceil \; (\forall s\in\services)$ and evaluated accuracy scores provided by PNNs $A_{s2} = \gamma^{\lambda_\text{pnn}} \cdot A_{s1} \; (\forall s\in\services)$ for the NN Special Case of the problem. For the experiments in our work, we set $\gamma=0.75$ and $\lambda_\text{pnn} = 0.75$.




\subsubsection{Split Neural Networks (SNNs)}
One approach to resource-conscious deep learning is split learning --- where a portion of a DNN's architecture is run on a resource-constrained device and the rest is run on a central server. The output of the last layer of a SNN's architecture is communicated from the resource-constrained device to the central server which finishes the final computation and communicates back the result~\cite{SL_2}. There are other arrangements for split learning, but this is the approach we adopt. For a comprehensive summary of split learning, refer to~\cite{vepakomma2018split}. We assume the architecture of a SNN largely matches its respective DNN and thus attaining near-equivalent accuracy. For these models, we consider a hyper-parameter $\rho\in(0,1)$ which correspond to the $\rho$-proportion of an SNN's respective DNN that is run/stored on an edge cloud and the remaining $(1-\rho)$-proportion that is run on the central cloud. 
For simplicity, service models where $m=3$ are considered as SNNs in this version of the MSIP problem. We also consider the storage capacity needed to store an SNN.
In short, in the SNN Special Case, let the number of layers $N^{s3} = \lceil \rho \cdot N^{s1} \rceil\; (\forall s \in\services)$.
%to be $\lceil\rho \cdot r_{s3}\rceil=r_{s1}\;(\forall s\in\services)$. 
Let storage costs $r_{s3} =  \lceil \rho \cdot r_{s1} \rceil \; (\forall s\in\services)$ and evaluated accuracy scores provided by SNNs $A_{s3} = \rho^{\lambda_\text{snn}} \cdot A_{s1} \; (\forall s\in\services)$ for the NN Special Case.
% \hana{why? didnt we assume accuracy provided by SNN is the same as DNN?}
For our experiments, we set $\rho=0.5$ and $\lambda_\text{snn} = 0.125$.
This setup makes accuracy for SNN models trained via split learning to be close to conventional DNNs trained via deep learning, while having an advantage over the pruned PNNs.
% {and $\rho=???$}. \nathaniel{$\rho$ is specified in the ``Parameter Setup" section.}






\subsection{ANN QoS Functions}
\label{sec:arch-QoS}
We explicitly define the expected completion times for the ANN models. Broadly speaking, we consider completion time of a request to be comprised of two processes: communication time delay and computation time delay. As such, we define the time delay function as follows,
\begin{equation}
	delay_{sm}(u) = delay_{sm}^{k}(u) + delay_{sm}^{w}(u)
\end{equation}
where the former term, $delay_{sm}^{k}(\cdot)$, is the communication delay function of service model~$(s,m)$ for user~$u$ and the latter term, $delay_{sm}^{w}(\cdot)$, is the computation delay function of service model~$(s,m)$ for user~$u$ and the latter term. 
%Both of these are defined as piecewise functions. In the case of the DNN and PNN, the definition is straightforward and identical to one another. The calculation performed for the DNN and PNN varies in that the PNN has a less complex architecture (i.e., less layers and neurons). The SNN model is more complicated for both cases, because only a portion of the architecture is run on the edge and the remaining portion is run on the cloud. As a result, there is additional incurred communication cost not found in the DNN and PNN models. 


\subsubsection{ANN Communication Delay}
\draft{For our experiments and without loss of generality, we consider each neuron in a service model's architecture to be represented as one bit.} We formally define the communication delay function below,
\begin{equation}
	delay_{sm}^{k}(u) =
	\begin{cases}
		\frac{\ell_1^{sm} + \ell_{N^{sm}}^{sm}}{bps_u} + \frac{\ell_{\lceil\rho\cdot N^{sm}\rceil}^{sm} + \ell_{N^{sm}}^{sm}}{bps_{c}/|\users_e|}  & m=3 \\
		% 
		\frac{1}{bps_u} (\ell_1^{sm} + \ell_{N^{sm}}^{sm}) & \text{otherwise}
	\end{cases}
	\label{eq:arch-comm-delay}
\end{equation}
where $bps_u$ is the two-way data transmission rate from user~$u$ to its edge cloud~$e_u$ and $bps_c$ is the data transmission rate from the edge cloud to the central cloud $c$ (we assume this is equal across all edge clouds). For simplicity, we assume that uplink and downlink are equivalent.
\draft{When $m=3$ (i.e., SNN), the communication delay is calculated as a communication from the user to and from their edge cloud, as well as to and from their edge cloud and the central cloud. $\ell_1^{sm}$ denotes the number of neurons in the first (or input) layer and $\ell_{N^{sm}}^{sm}$ denotes the number of neurons in the last (or output layer) --- these are communicated to and from the user and edge cloud. Then $\ell^{sm}_{\lceil\rho\cdot N^{sm}\rceil}$ represents the number of neurons in last layer on the edge cloud that is communicated to the central cloud for processing (in addition to the results of the output layer being communicated back to the edge cloud). When $m\neq3$, we only consider the first layer and last layer of the architecture with no communication to the central cloud.}
The formulation for Eq.~\eqref{eq:arch-comm-delay} is based on the necessary amount of input and output data for a given service model $(s,m)$. The number of neurons in the input layer (denoted by $\ell_1^{sm}$) can be thought of as the size of the input/output data. 
In the special case of the MSIP problem, we consider each user to have additional parameters to calculate their data transmission rate. First, we consider that each user has a distance from the edge cloud $dist_u\;(\forall u\in\users)$. Additionally, we consider a maximal distance value $dist_{\max}$ to be the greatest for an edge cloud to establish a connection, thus $dist_u \leq dist_{\max}\;(\forall u\in\users)$. With this said, we consider the data transmission rate (bits-per-second) for user~$u$ to its edge cloud to be 
$bps_u = (K_e/|\users_e|) \cdot \log_2(1 + \frac{dist_{\max}-dist_u}{dist_{\max}})$ with $K_e$ being in Hz.
% \hana{what do you mean by in Hz? Isn't the $bps_{u}$ in bits/sec? do you mean $K_e$ is in Hz? bit reading this sentence i dont get that impression. clarify} \nathaniel{Better?} 
This definition is largely based on the Shannon-Hartley Theorem~\cite{shannon_hartley} with the distance portion relating to signal-to-noise ratio. We make these considerations due to the fact that the input size for PNNs vary from that of DNNs and SNNs.

\subsubsection{ANN Computation Delay}
Finally, we formally define the computation delay function below in Eq.~\eqref{eq:arch-comp-delay} as,
\begin{equation}
	delay_{sm}^{w}(u) =
	\begin{cases}
		\frac{1}{W_{e_u}/|\users_{e_u}|}  \sum_{i=1}^{\lceil\rho\cdot N^{sm}\rceil} (\ell_i^{sm}\beta_i^{sm}) & m=3 \\
		%		
		\frac{1}{W_{e_u}/|\users_{e_u}|} (\ell^{sm}\cdot\beta^{sm}) & \text{otherwise.}
	\end{cases}
	\label{eq:arch-comp-delay}
\end{equation}

\noindent \draft{When $m\neq3$, we can compute the computation delay by computing the number of CPU clock cycles necessary to run the service model and then simply dividing that by the user's share of its edge cloud's computational resources (i.e., $1/(W_{e_u}/|\users_{e_u}|)$). To compute a DNN or PNN's number of needed CPU clock cycles, we simply need to perform the dot product of its $\ell^{sm}$ and $\beta^{sm}$ vectors --- with the former representing the number of neurons in each layer and the latter representing the number of CPU cycles needed for each neuron using its activation function. For SNNs (i.e., $m=3$), we only consider computation delay on the edge cloud. We assume the central cloud's computational resources to be sufficient enough to provide negligible delay due to computation --- meaning incurred cost for communicating with the central cloud is due to communication. We essentially perform a dot product for the architecture portion stored on the edge cloud (i.e., $\sum_{i=1}^{\lceil\rho\cdot N^{sm}\rceil}(\ell_i^{sm}\beta_i^{sm})$).
}



\subsection{ANN Special Case Objective Function}
The goal of this work is to maximally place service models on the edge cloud such that its utility is optimal. In other words, we aim to minimize the edge cloud's reliance on the central cloud, if possible, while attaining near-optimal QoS. That being said, the model type of SNN poses a problem. SNNs are inherently reliant on the central cloud to perform inference. As a result, there should be some associated cost. As such, we adjust the objective function $Z$ provided in Eq.~\eqref{eq:objective} to be the following for NN experiments,
\begin{multline}
	Z = 
	\sum_{e\in\edges} \sum_{u\in\users_e} 
	\Bigg(
		\sum_{m\in\model}
		y_u^m\; QoS(u, s_u, m; \Delta)
	    - \\
    	\Big(
    		\theta y_u^m QoS(u, s_u, m; \Delta) I_{(m=3)}
    	\Big)
	\Bigg).
%	- \theta y_u^3 QoS(u, s_u, 3).
%	
	\label{eq:arch-MSIP}
\end{multline}
In Eq.~\eqref{eq:arch-MSIP}, we include an additional hyper-parameter, $\theta$, which represents the \emph{cost} (e.g., monetary, computational, etc.) associated with using the central cloud in case of the SNNs to service user requests. Additionally, we consider an indicator function $I_{(m=3)}$ which is equal to $1$ when $m=3$, and 0 otherwise. This is used to only induce penalty based on $\theta$ for scheduled SNN models. For this work, we set $\theta=0.05$.
% \hana{what is the value of$\theta$ for the experiments?}
